TimePFN: Effective Multivariate Time Series Forecasting with Synthetic Data

The diversity of time series applications and scarcity of domain-specific data highlight the need for time-series models with strong few-shot learning capabilities. In this work, we propose a novel training scheme and a transformer-based architecture, collectively referred to as TimePFN, for multivariate time-series (MTS) forecasting. TimePFN is based on the concept of Prior-data Fitted Networks (PFN), which aims to approximate Bayesian inference. Our approach consists of (1) generating synthetic MTS data through diverse Gaussian process kernels and the linear coregionalization method, and (2) a novel MTS architecture capable of utilizing both temporal and cross-channel dependencies across all input patches. We evaluate TimePFN on several benchmark datasets and demonstrate that it outperforms the existing state-of-the-art models for MTS forecasting in both zero-shot and few-shot settings. Notably, fine-tuning TimePFN with as few as 500 data points nearly matches full dataset training error, and even 50 data points yield competitive results. We also find that TimePFN exhibits strong univariate forecasting performance, attesting to its generalization ability. Overall, this work unlocks the power of synthetic data priors for MTS forecasting and facilitates strong zero- and few-shot forecasting performance.

==> figures/fig_spider.tex <==
\begin{figure}[t!] 
   \centering    \includegraphics[width= 0.45\textwidth]{spider_plot.pdf}
   \caption{Average forecasting performance (MSE) of TimePFN. MSE values are averaged over all data budgets. }
    %in the example - the one above is an acyclic graph while the other graph contains a cycle. For each sub-graph, we calculate the strongly connected components. According to Definition \ref{cyc sub}, we derive $\bdata$ based on $\data$ as shown in the right figure. In other words, the graphs are reduced to non-singleton SCCs. As a result, $\Gc^{(1)}$ is removed from the dataset.   \label{fig:main_figure}
\end{figure}

==> figures/fig_timePFN.tex <==
\begin{figure}[t!] 
   \centering    \includegraphics[width= 0.47\textwidth]{figures/timePFN.pdf}
   \caption{Illustration of the architecture of TimePFN. Variates are filtered with 1D convolutions, to be patched with overlapping strides, following \cite{Yuqietal-2023-PatchTST}. They are then fed into transformer encoder with channel mixing, with the final forecast coming from the final feedforward network.}
    %in the example - the one above is an acyclic graph while the other graph contains a cycle. For each sub-graph, we calculate the strongly connected components. According to Definition \ref{cyc sub}, we derive $\bdata$ based on $\data$ as shown in the right figure. In other words, the graphs are reduced to non-singleton SCCs. As a result, $\Gc^{(1)}$ is removed from the dataset.   \label{fig:main_figure}
\end{figure}

==> tables/architectural_ablations.tex <==

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{0.3mm}
\begin{tabular}{ll|lr|rl|rl|rl|rl|rl|rl|ll|ll}
\hline
\multicolumn{2}{c|}{Dataset} & \multicolumn{2}{c|}{ECL} & \multicolumn{2}{c|}{Weather} & \multicolumn{2}{c|}{Traffic} & \multicolumn{2}{c|}{Solar-Energy} & \multicolumn{2}{c|}{Exchange} & \multicolumn{2}{c|}{ETTh1} & \multicolumn{2}{c|}{ETTh2} & \multicolumn{2}{c|}{ETTm1} & \multicolumn{2}{c}{ETTm2} \\ \cline{3-20} 
\multicolumn{2}{c|}{Models} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\ \hline
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{z.s. }}} & TimePFN & \textbf{0.315} & \textbf{0.383} & \textbf{0.209} & \textbf{0.255} & \textbf{1.108} & \textbf{0.613} & \textbf{0.941} & \textbf{0.730} & \textbf{0.105} & \textbf{0.229} & \textbf{0.453} & \textbf{0.439} & 0.328 & \textbf{0.362} & \textbf{0.637} & \textbf{0.512} & \textbf{0.212}  & \textbf{0.291} \\
 &TimePFN-w/o Conv & 0.653 & 0.637 & 0.221 & 0.271 & 1.287 & 0.757 & 1.197 & 0.829 & 0.111 & 0.237 & 0.608 & 0.517 & 0.338 & 0.374  & 0.771 & 0.565 & 0.224 & 0.307 \\ 
  & PatchTST-PFN & 0.470 & 0.522 & 0.212 & 0.262 & 1.172 & 0.702 & 1.014 & 0.787 & 0.108 & 0.231 & 0.554 & 0.501 & \textbf{0.322} & 0.366  & 0.746 & 0.560 & 0.215 & 0.301 \\  \hline


\end{tabular}
\caption{In TimePFN-w/o-Convolution, we eliminate the convolutional operator that is normally applied to the initial input variates. In PatchTST-PFN, we train a PatchTST model to evaluate the significance of channel-mixing and the appropriateness of our architecture for PFNs. Both the sequence length and the forecasting length are set to 96. }
\label{tbl:arch-ablation}
\end{table*}

==> tables/data_ablation.tex <==

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{0.3mm}
\begin{tabular}{ll|lr|rl|rl|rl|rl|rl|rl|ll|ll}
\hline
\multicolumn{2}{c|}{Dataset} & \multicolumn{2}{c|}{ECL} & \multicolumn{2}{c|}{Weather} & \multicolumn{2}{c|}{Traffic} & \multicolumn{2}{c|}{Solar-Energy} & \multicolumn{2}{c|}{Exchange} & \multicolumn{2}{c|}{ETTh1} & \multicolumn{2}{c|}{ETTh2} & \multicolumn{2}{c|}{ETTm1} & \multicolumn{2}{c}{ETTm2} \\ \cline{3-20} 
\multicolumn{2}{c|}{Models} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\ \hline
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{z.s. }}} & TimePFN & \textbf{0.315} & \textbf{0.383} & \textbf{0.209} & \textbf{0.255} & \textbf{1.108} & \textbf{0.613} & \textbf{0.941} & \textbf{0.730} & \textbf{0.105} & \textbf{0.229} & \textbf{0.453} & \textbf{0.439} & 0.328 & \textbf{0.362} & \textbf{0.637} & \textbf{0.512} & \textbf{0.212}  & \textbf{0.291} \\
 &TimePFN-Ind & 0.350 & 0.416 & 0.214 & 0.260 & 1.180 & 0.651 & 1.197 & 0.829 & 0.113 & 0.238 & 0.468 & 0.447 & \textbf{0.326} & 0.363  & 0.761 & 0.542 & 0.215 & 0.295 \\  \hline


\end{tabular}
\caption{TimePFN-ind is the model trained using only independent variates, while the other model is our standard one, which we used throughout the experiments. Both models have a sequence and forecasting length of 96. }
\label{tbl:data-ablation}
\end{table*}




==> tables/main_table.tex <==

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{0.6mm}
\begin{tabular}{ll|lr|rl|rl|rl|rl|rl|rl|ll|ll}
\hline
\multicolumn{2}{c|}{Dataset} & \multicolumn{2}{c|}{ECL} & \multicolumn{2}{c|}{Weather} & \multicolumn{2}{c|}{Traffic} & \multicolumn{2}{c|}{Solar-Energy} & \multicolumn{2}{c|}{Exchange} & \multicolumn{2}{c|}{ETTh1} & \multicolumn{2}{c|}{ETTh2} & \multicolumn{2}{c|}{ETTm1} & \multicolumn{2}{c}{ETTm2} \\ \cline{3-20} 
\multicolumn{2}{c|}{Models} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\ \hline
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{z.s. }}} & TimePFN & \textbf{0.315} & \textbf{0.383} & \textbf{0.209} & \textbf{0.255} & \textbf{1.108} & \textbf{0.613} & 0.941 & \textbf{0.730} & 0.105 & 0.229 & \textbf{0.453} & \textbf{0.439} & \textbf{0.328} & \textbf{0.362} & \textbf{0.637} & \textbf{0.512} & \textbf{0.212}  & \textbf{0.291} \\
 & Naive & 1.587 & 0.945 & 0.259 & 0.254 & 2.714 & 1.077 & 1.539 & 0.815 & \textbf{0.081} & \textbf{0.196} & 1.294 & 0.713 & 0.431 & 0.421  & 1.213 & 0.664 & 0.266 & 0.327 \\ 
  & SeasonalNaive & 1.618 & 0.964 & 0.268 & 0.263 & 2.774 & 1.097 & 1.599 & 0.844 & 0.086 & 0.204 & 1.325 & 0.727 & 0.445 & 0.431  & 1.227 & 0.673 & 0.274 & 0.334 \\ 
  & Mean & 0.845 & 0.761 & 0.215 & 0.271 & 1.410 & 0.804 & \textbf{0.910} & 0.734 & 0.139 & 0.269 & 0.700 & 0.558 & 0.352 & 0.387 & 0.693 & 0.547 & 0.229 & 0.307 \\ \hline \hline
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Budget =50 }}} & TimePFN & \textbf{0.235} & \textbf{0.322} & \textbf{0.190} & \textbf{0.235} & \textbf{0.746} & \textbf{0.468} & \textbf{0.429} & \textbf{0.450} & \textbf{0.096} & \textbf{0.218}  & \textbf{0.438} & \textbf{0.429} & \textbf{0.324} & \textbf{0.359} &  \textbf{0.419} & \textbf{0.418} & \textbf{0.195} & \textbf{0.276} \\
 & iTransformer & 0.278 & 0.360 & 0.237 & 0.278 & 0.801 & 0.499 & 0.513 & 0.479  & 0.145 & 0.275 & 0.838 & 0.617 & 0.410 & 0.422  & 0.884   & 0.608  & 0.268 & 0.337 \\
 & PatchTST & 0.667 & 0.646 & 0.221 & 0.269 & 1.295 & 0.746 & 0.810 & 0.669 & 0.127 & 0.255 & 0.778 & 0.587 & 0.372 & 0.401 & 0.656 & 0.528 & 0.231 & 0.310 \\
 & DLinear & 0.406 & 0.463 & 0.742 & 0.612 & 1.888 & 0.937 & 0.956 & 0.813 & 3.432 & 1.349 & 1.404 & 0.881 & 3.928 & 1.383 & 1.332 & 0.846 & 3.484 & 1.290 \\
 & FEDFormer & 0.908 & 0.758 & 0.306 & 0.381 & 1.587 & 0.874 & 0.972 & 0.757 & 0.165 & 0.300 & 0.676 & 0.570 & 0.424 & 0.468  & 0.745 & 0.589 & 0.291 & 0.387 \\ 
& Informer & 1.226 & 0.896 & 0.464 & 0.511 & 1.714 & 0.901 & 0.887 & 0.783 & 1.470 & 1.007 & 1.172 & 0.819 & 2.045 & 1.093  & 1.003 & 0.745 & 1.590 & 0.995 \\ 
  & Autoformer & 0.729 & 0.675 & 0.322 & 0.401 & 1.600 & 0.883 & 1.065 & 0.808 & 0.213 & 0.351 & 0.607 & 0.560 & 0.492 & 0.506 & 0.763 & 0.592 & 0.316 & 0.407 \\ \hline \hline


  

\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Budget =500 }}} & TimePFN & \textbf{0.190} & \textbf{0.283} & \textbf{0.178} & \textbf{0.222} & \textbf{0.487} & \textbf{0.335} & \textbf{0.269} & \textbf{0.305} & 0.083 & 0.203 & \textbf{0.401} & \textbf{0.412} & \textbf{0.311} & \textbf{0.352} & \textbf{0.360} & \textbf{0.386} & \textbf{0.185} & \textbf{0.268} \\
 & iTransformer & 0.200 & 0.284 & 0.211 & 0.248 & 0.514 & 0.354  & 0.307 & 0.334 & 0.113 & 0.239 & 0.489 & 0.470 & 0.361 & 0.394 & 0.569 & 0.494 & 0.231 & 0.310  \\
 & PatchTST & 0.236 & 0.320 & 0.210 & 0.246 & 0.740 & 0.455 & 0.321 & 0.353 & \textbf{0.081} & \textbf{0.198} & 0.596 & 0.515 & 0.358 & 0.392 & 0.369  & 0.386 & 0.190 & 0.275  \\
 & DLinear & 0.235 & 0.328 & 0.335 & 0.394 & 1.312 & 0.727 & 0.622 & 0.656 & 0.655 & 0.551 & 0.749 & 0.609 & 1.098 & 0.712 & 0.817 & 0.621 & 0.870 & 0.626 \\
 & FEDformer & 0.317 & 0.407 & 0.265 & 0.341 & 0.888 & 0.548 & 0.821 & 0.706 & 0.157 & 0.288 & 0.444 & 0.452 & 0.358 & 0.401  & 0.674 & 0.542 & 0.238 & 0.322 \\ 
   & Informer & 0.869 & 0.760 & 0.320 & 0.393 & 1.411 & 0.774 & 0.318 & 0.385 & 0.699 & 0.694 & 0.913 & 0.713 & 1.311 & 0.940  & 0.704 & 0.595 & 1.121 & 0.803 \\ 
  & Autoformer & 0.303 & 0.396 & 0.237 & 0.312 & 0.896 & 0.549 & 0.950 & 0.787 & 0.158 & 0.290 & 0.456 & 0.456 & 0.339 & 0.384 & 0.672 & 0.534 & 0.223 & 0.308 \\ \hline \hline




  
 \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Budget = All }}} & TimePFN & \textbf{0.138} & \textbf{0.137} & \textbf{0.166} & \textbf{0.208} & \textbf{0.392} & \textbf{0.260} & 0.203 & 0.219 & 0.100 & 0.223 & 0.402 & 0.417 & \textbf{0.293} & \textbf{0.343} & 0.392 & 0.402 & 0.180 & 0.262 \\
 & iTransformer & 0.147 & 0.239 & 0.175 & 0.215  & 0.393 & 0.268 & 0.201 & 0.233 & 0.086& 0.206  & \textbf{0.387} & 0.405 & 0.300 & 0.349 & 0.342 & 0.376 & 0.185 & 0.272 \\
 & PatchTST & 0.185 & 0.267 & 0.177 & 0.218 & 0.517 & 0.334 & 0.222 & 0.267 & \textbf{0.080} & \textbf{0.196} & 0.392 & \textbf{0.404} & \textbf{0.293} & \textbf{0.343} & \textbf{0.318} & \textbf{0.357} & \textbf{0.177} & \textbf{0.260} \\
 & DLinear & 0.195 & 0.278 & 0.341 & 0.412 & 0.690 & 0.432 & 0.286 & 0.375 & 0.101 & 0.237 & 0.400 & 0.412 & 0.357 & 0.406  & 0.344 & 0.371 & 0.195 & 0.293 \\
 & FEDformer & 0.196 & 0.310 & 0.227 & 0.313 & 0.573 & 0.357 & 0.242 & 0.342 & 0.148 & 0.280 & 0.380 & 0.417 & 0.340 & 0.386  & 0.363 & 0.408 & 0.191 & 0.286 \\ 
& Informer & 0.327 & 0.413 & 0.455 & 0.481 & 0.735 & 0.409 & \textbf{0.190} & \textbf{0.216} & 0.921 & 0.774 & 0.930 & 0.763 & 2.928 & 1.349  & 0.623 & 0.559 & 0.396 & 0.474 \\ 
  & Autoformer & 0.214 & 0.327 & 0.273 & 0.344 & 0.605 & 0.376 & 0.455 & 0.480 & 0.141 & 0.271 & 0.440 & 0.446 & 0.364 & 0.408 & 0.520 & 0.490 & 0.233 & 0.311 \\ \hline 
\multicolumn{2}{c|}{\# of Variates} & \multicolumn{2}{c|}{321} & \multicolumn{2}{c|}{21} & \multicolumn{2}{c|}{862} & \multicolumn{2}{c|}{137} & \multicolumn{2}{c|}{8} & \multicolumn{2}{c|}{7} & \multicolumn{2}{c|}{7} & \multicolumn{2}{c|}{7} & \multicolumn{2}{c}{7} \\ 

\end{tabular}
\caption{MTS forecasting results of TimePFN and comparable architectures with best results in bold. Input and prediction lengths are set to be 96. \name demonstrates remarkable performance in budget-limited settings, as well as with the full dataset, particularly in scenarios involving a large number of variates.}
\label{tbl:mse_main}
\end{table*}


==> tables/univariate_tables.tex <==
\begin{table*}[ht]
\small
\setlength{\tabcolsep}{0.9mm}
\begin{center}

\begin{tabular}{ll|lr|rl|rl|rl|rl|rl|rl|ll|}
\hline
\multicolumn{2}{c|}{Dataset} & \multicolumn{2}{c|}{TimePFN-36} & \multicolumn{2}{c|}{TimePFN-96} & \multicolumn{2}{c|}{ForecastPFN} & \multicolumn{2}{c|}{Chronos-s}  & \multicolumn{2}{c|}{SeasonalN.} & \multicolumn{2}{c|}{Naive} & \multicolumn{2}{c|}{Mean} \\ \cline{3-16} 
\multicolumn{2}{c|}{Models} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE  \\ \hline
\multicolumn{2}{l|}{ECL} & \textbf{0.752} & \textbf{0.703} & 0.509 & 0.549 & 1.416 & 0.958 & 1.152 & 0.792  & 1.559  & 0.995 & 1.211 & 0.829  &0.963  & 0.805   \\
\multicolumn{2}{l|}{Weather$\times 10^{2}$} & 0.042 &   1.381 & 0.046 & 1.477 & 0.084 & 1.999 & 0.036 & 1.136   &0.045 & 1.352  & \textbf{0.035}  & \textbf{1.123}  & 0.069  & 1.893  \\
\multicolumn{2}{l|}{Traffic} & \textbf{1.503} & \textbf{1.032} & 0.414 & 0.503 &4.521 & 1.742 & 3.103 & 1.364   &4.301  & 1.771 & 3.330  &1.463  & 2.125 & 1.256   \\ 
\multicolumn{2}{l|}{Exchange} & 0.027 & 0.125 & 0.034 & 0.139 & 0.057 & 0.180 & 0.049 & 0.113 & 0.028 & 0.128 & \textbf{0.022} & \textbf{0.107} & 0.040 & 0.156   \\ 
\multicolumn{2}{l|}{ETTh1} & \textbf{0.029} & 0.130 & 0.030 & 0.133 & 0.102 & 0.237 & 0.061 & 0.155  &  0.039& 0.151 & 0.031 & \textbf{0.128} & 0.040 & 0.154  \\ 
\multicolumn{2}{l|}{ETTh2} & \textbf{0.126} & \textbf{0.273} & 0.086 & 0.224 & 0.434 & 0.517  & 0.207 & 0.321  &0.279& 0.408 &0.215  & 0.336 &0.168  & 0.321  \\ \hline 

\end{tabular}

\end{center}
\caption{Zero-shot results of TimePFN on univariate time-series forecasting with input length = 36. TimePFN-96 has input length of 96. The errors are averaged over forecasting lengths of $\{6,8,14,18,24,36,48\}$. Chronos-s stands for Chronos-small. The best results are in bold (excluding TimePFN-96). } 
\label{tbl:univariate_res}
\end{table*}

